Revisiting ResNets: Improved Training and Scaling Strategies

Novel computer vision architectures monopolize the spotlight, but the impact of the model architecture is often conflated with simultaneous changes to training methodology and scaling strategies. Our work revisits the canonical ResNet (He et al., 2015) and studies these three aspects in an effort to disentangle them. Perhaps surprisingly, we find that training and scaling strategies may matter more than architectural changes, and further, that the resulting ResNets match recent state-of-the-art models. We show that the best performing scaling strategy depends on the training regime and offer two new scaling strategies: (1) scale model depth in regimes where overfitting can occur (width scaling is preferable otherwise); (2) increase image resolution more slowly than previously recommended (Tan & Le, 2019). Using improved training and scaling strategies, we design a family of ResNet architectures, ResNet-RS, which are 1.7x - 2.7x faster than EfficientNets on TPUs, while achieving similar accuracies on ImageNet. In a large-scale semi-supervised learning setup, ResNet-RS achieves 86.2% top-1 ImageNet accuracy, while being 4.7x faster than EfficientNet NoisyStudent. The training techniques improve transfer performance on a suite of downstream tasks (rivaling state-of-the-art self-supervised algorithms) and extend to video classification on Kinetics-400. We recommend practitioners use these simple revised ResNets as baselines for future research.

==> sections/old/old.tex <==
% \begin{tabular}{l|l|rr}
%   \hline
%   Model & Regularization & WD = 1e-4 & WD = 4e-5 \\
%   \hline
%   ResNet-50 & None & 77.2 & \textcolor{red}{(-1.5)} 75.7 \\
%   ResNet-50 & RA + LS & 80.0 & (0.0) 80.0 \\
%   %ResNet-50 & RA + LS + SD + DO & 79.0 & \textcolor{blue}{(+0.6)} 79.6 \\
%   ResNet-50 & RA + LS + DO & 79.7 & \textcolor{blue}{(+0.6)} \textbf{80.3} \\
%   \hline
%   ResNet-200 & None & 80.1 & \textcolor{red}{(-0.4)} 79.7 \\
%   ResNet-200 & RA + LS & 83 & \textcolor{red}{(-0.5)} 82.5  \\
%   ResNet-200 & RA + LS + SD + DO & 83.3 & \textcolor{blue}{(+0.3)} \textbf{83.6} \\
%   \hline
% \end{tabular}

% \begin{table*}[ht!]
% \centering
% \begin{tabular}{llcccc}
%   \toprule
%   Model & Loss & Augmentation & Labels & Epochs & Imagenet Accuracy \\
%   \midrule
%   %ResNet-50 & Supervised Contrastive loss & \checkmark & \checkmark & 700 & 78.8 \\
%   %ResNet-50 & Improved Supervised Training & \checkmark & \checkmark & 350 & 78.4 \\
%   %ResNet-50 & Best we can get & \checkmark & \checkmark & 350 & \todo{} \\
%   %\midrule
%   ResNet-200 & Baseline Supervised Training \cite{khosla2020supervised} & \checkmark & \checkmark & 700 & 78.8 \\
%   ResNet-200 & Supervised Contrastive loss \cite{khosla2020supervised} & \checkmark & \checkmark & 700 & 80.8 \\
%   ResNet-200 & Improved Supervised Training & \checkmark & \checkmark & 350 & \textbf{81.5} \\
%   %ResNet-200 & Best we can get & \checkmark & \checkmark & 350 & \todo{} \\
%   \bottomrule
% \end{tabular}
% \caption{Our improved training methodology outperforms the supervised contrastive loss~\cite{khosla2020supervised} despite training for half the number of iterations.\todo{Any other papers with shaky baselines that we could reference here?}}
% \label{tab:supervised_constrastive} 
% \end{table*}


\iffalse

\newcommand{\improv}[1]{\textcolor{blue}{(+#1)}}
\begin{table*}[h!]
\centering
\begin{tabular}{lrrr}
  \hline
  Model & Image Size & Epochs & Top-1  \\
  \hline
  ResNet-50 & 224 & 100 & 76.9  \\
  ResNet-50-SE & 224 & & \improv{1.0} 77.9  \\
  ResNet-50-SE-D & 224 & & \improv{0.6} 78.5  \\
  \hline
  ResNet-50 & 224 & 200 & 77.9  \\
  ResNet-50-SE & 224 & & \improv{1.0} 78.9  \\
  ResNet-50-SE-D & 224 & & \improv{0.6} 79.5  \\
  \hline
  ResNet-50 & 224 & 400 & 78.6  \\
  ResNet-50-SE & 224 & & \improv{1.1} 79.7  \\
  ResNet-50-SE-D & 224 & & \improv{0.5} 80.2  \\
  \hline
  ResNet-50 & 448 & 400 & 79.9 \\
  ResNet-50-SE & 448 & & \improv{1.1} 81.0 \\
  ResNet-50-SE-D & 448 & & \improv{0.4} 81.4 \\
  \hline
  ResNet-152 & 224 & 400 & 81.4  \\
  ResNet-152-SE & 224 & & \improv{0.2} 81.6  \\
  ResNet-152-SE-D & 224 & & \improv{0.6} 82.2  \\
  \hline
  ResNet-152 & 448 & 400 & 82.5  \\
  ResNet-152-SE & 448 & & \improv{0.7} 83.2  \\
  ResNet-152-SE-D & 448 & & \improv{0.0} 83.2  \\
\end{tabular}
\caption{Architecture changes/tricks matter less when models are larger, and a strong setup is used.}
\label{tab:architectural_components} 
\end{table*}


\begin{table*}[h!]
\centering
\begin{tabular}{l|rrrrrr|r}
  \hline
  Model & 100 Epochs & 200 Epochs & 400 Epochs & 600 Epochs  \\
  \hline
  ResNet-50 & \\
  ResNet-101 & \\
  ResNet-152 &\\
\end{tabular}
\caption{Impact of training iterations on model performance.}
\label{tab:ResNet Performance} 
\end{table*}


\begin{table}[h]
\centering
\begin{tabular}{l|r|r|r}
  \hline
  Model & Image Size & Top 1 Acc & TPU Speed \\
  \hline
  ResNet-50 & 224 &  & \\
  ResNet-SE-50 & 224 & &   \\
  ResNet-D-SE-50 & 224 & &  \\
  ResNet-D-SE-50 & 352 & &  \\
  ResNet-D-SE-50 & 480 & &  \\
  \hline
  ResNet-101 & 224 &  & \\
  ResNet-SE-101 & 224 & & \\
  ResNet-D-SE-101 & 224 & & \\
  ResNet-D-SE-101 & 352 & & \\
  ResNet-D-SE-101 & 480 & & \\
  \hline
  ResNet-152 & 224 &  &  \\
  ResNet-SE-152 & 224 & & \\
  ResNet-D-SE-152 & 224 & & \\
  ResNet-D-SE-152 & 352 & & \\
  ResNet-D-SE-152 & 480 & & \\
  \hline
\end{tabular}
\caption{}
\label{tab:ResNet Performance} 
\end{table}

\begin{table*}[h!]
\centering
\begin{tabular}{l|r|rrrr}
  \hline
  Model & ImageNet Top-1 & AP 12 Ep & AP 24 Ep & AP 36 Ep & AP 72 Ep  \\
  \hline
  ResNet-50 (Supervised) & 76.5 &   \\
  ResNet-50 (SimCLR) & --- &  \\
  ResNet-50 (Supervised) & 78.9 &   \\
\end{tabular}
\caption{Transfer learning performance on COCO with different ResNet-50 checkpoints. 1024 images.}
\label{tab:ResNet Performance} 
\end{table*}

\begin{table*}[h!]
\centering
\begin{tabular}{l|rrrr|r}
  \hline
  Model & LS & LS + RA & LS + RA + SD & LS + RA + SD + DO & Top-1  \\
  \hline
  WD=1e-4 & \\
  WD=5e-4 & \\
\end{tabular}
\caption{Ablation of commonly used training tricks.}
\label{tab:ResNet Performance} 
\end{table*}

\fi




\begin{table}[ht!]
\centering
\begin{tabular}{lcc}
  \toprule
  Model & Epochs & ImageNet Acc \\
  \midrule
  ResNet-152 & 90 & 78.6 \\
  ResNet-152 w/ Tuning & 400 & 81.6 \\
  ResNet-152 (best we can get) & 400 & \todo{} \\
  ResNet-152 SimCLR V2 & 800 & 79.3 \\
  ResNet-152 SimCLR V2 (FT) & 1200 & ??? \\
  \midrule
  ResNet-152 2x & 90 & 79.3 \\
  ResNet-152 2x w/ Tuning & 400 & 83.2 \\
  ResNet-152 2x (best we can get) & 400 & \todo{} \\
  ResNet-152 2x SimCLR V2 & 800 & 81.1 \\
  ResNet-152 2x SimCLR V2 (FT) & 1200 & ??? \\
  \bottomrule
\end{tabular}
\caption{Supervised training strongly outperforms unsupervised contrastive pretraining and supervised fine-tuning (SimCLR V2 fine-tuned on 100\% of ImageNet labels).}
\label{tab:imagenet_transfer}
\end{table}


\begin{table*}[t!]
\centering
\begin{tabular}{lllllll}
  \hline
  Model & Year & Image Size & Epochs & Regularization & WD & ImageNet Top-1 \\
  \hline
  AlexNet & 2012 & & & & & \\
  ResNet (original) \\
  ResNet (Cloud TPU) \\
  SENet? Inception-ResNetv2? Pyramid ResNet \\
  EfficientNet & & 224-680? & &  \\
  TResNet & & 224-448 & &  \\
  ResNeSt & & 224-416 & &  \\
  ResNet (ours)
\end{tabular}
\caption{Training methodologies used in state-of-the-art classification models. Training methodologies has significantly evolved over the years and explains most improvements in ImageNet accuracy. Models that were trained using extra training data or pre/post-processing are excluded. \todo{The goal of this table to showcase how improvements were largely driven by training longer, augmentation and larger images. Organize by year. Check https://openai.com/blog/ai-and-efficiency/ for inspiration} \todo{Include GoogLeNet?}}
\label{tab:training_setups} 
\end{table*}
